Testing the Agreement of Trees with Internal Labels

The input to the agreement problem is a collection $P = \{T_1, T_2, \dots , T_k\}$ of phylogenetic trees, called input trees, over partially overlapping sets of taxa. The question is whether there exists a tree $T$, called an agreement tree, whose taxon set is the union of the taxon sets of the input trees, such that for each $i \in \{1, 2, \dots , k\}$, the restriction of $T$ to the taxon set of $T_i$ is isomorphic to $T_i$. We give a $O(n k (\sum_{i \in [k]} d_i + \log^2(nk)))$ algorithm for a generalization of the agreement problem in which the input trees may have internal labels, where $n$ is the total number of distinct taxa in $P$, $k$ is the number of trees in $P$, and $d_i$ is the maximum number of children of a node in $T_i$.

==> sections/subsections/analysis.tex <==
% !TEX root = ../../main.tex
\subsection{Correctness}

\begin{theorem}
\BuildAST (i) correctly builds up an agreement tree \T\ if input profile $\P= \{\T_1, \T_2, \dots , \T_k\}$ agrees, otherwise (ii) terminates immendiately.
\end{theorem}

\begin{proof}
To prove this theorem, we firstly show that only fully exposed labels in a position $\pi$ need to be removed. Obviously, for any node $\pi_i$ where $\ell \in \pi_i$ is not fully exposed, there must exist another tree $\T_j$ and a node $u \in V(\T_j)$, such that $\ell \in u$ and $u \in \Desc(\pi_j)$. By definition of agreement tree and LCA mappings, the parent-child relationships between $\pi_i$ and $Ch_{\T_i}(\pi_i)$ must be preserved. This indicates that all labels that are not fully exposed may not need to be processed. Clearly, if $\pi_i$ for every $i \in [k]$ is not fully exposed, this implies that the profile $\P$ does not agree and no label in $\pi$ will be processed. Therefore, \BuildAST\ should terminate immediately(Line \ref{algo:nolabel} in Algorithm \ref{algo:buildast}).

Now we assume that there exists a set $L$ of nodes from $\pi$ that are fully exposed. Let $\mathcal{W}$ be a collection of connected components resulted from deleting these nodes. (i) $|\mathcal{W}| = 0$. It is straightforward that $\pi$ should include a single leaf node, and the successor of such a position $\pi$ is \NULL. Thus all three conditions (C1 -- C3) are satisfied automatically. (ii) $|\mathcal{W}| \ge 1$. (a) If for each $W \in \mathcal{W}$, $|child_i(W)| \leq 1$ for $i \in [k]$, then condition C1 holds true immediately. Let $S = L$ under this condition, then every $\ell \in L(\pi) \setminus S$ is $\ell$ that is not fully exposed. As they are not removed from the graph so far, then there must exist a connected component $W' \in \mathcal{W}$ such that $Ch_{\T_i}(\pi_i) \in V(W')$ where $\ell \in \pi_i$. This implies that condition C2 is preserved. Since $Ch_\P(\pi) = \bigcup_{i \in [k]}Ch_{\T_i}(\pi_i)$, then $Ch_\P(\pi) = \bigcup_{W \in \mathcal{W}}(\bigcup_{i \in [k]}child_i(W))$. Let $A^W = \bigcup_{i \in [k]}child_i$ for each $W \in \mathcal{W}$, then $\Gamma = \bigcup_{W \in \mathcal{W}}A^W$ satisfies the condition C3 and thus $L$ includes all (strictly) semi-universal nodes. By Lemma \ref{lemma:iffstatement}, if there exists an agreement tree for $\pi$, then each position $\pi^{A^W}$ has an agreement tree. Line \ref{algo:singlecomponent} in Algorithm \ref{algo:buildast}(or Algorithm \ref{algo:singlefunction}) would handle this case. (b) If there exists $W \in \mathcal{W}$ such that $|child_i(W)| \ge 2$ or a subset $\mathcal{U} \subseteq \mathcal{W}$ such that $|Ch_{\T_i}(\pi_i) \cap V(\mathcal{U})| \ge 2$ for some $i$, it is clearly that in both cases $\ell \in \pi_i$ violates the condition C1, then $\ell \in \pi_i$ cannot be in $S$ where $S \subseteq L$. By definition of agreement tree and LCA mappings, for each such index $i$, $Ch_{\T_i}(\pi_i)$ should be in the same set $A^r \in \Gamma$. Due to this, all components $W \in \mathcal{W}$ that include $Ch_{\T_i}(\pi_i)$ should be grouped together. This approach results a larger set $A^r$, and there might be new labels $\ell' \in \pi_j$ violating condition C1. This process is repeated until no new label $\ell'' \in \pi_{j'}$ violates condition C1.  These labels together with non-fully exposed labels meet the requirement of condition C2 and the rest of the labels left in $L$ satisfy condition C1. Due to corresponding groups of components are disjoint mutually, then condition C3 is preserved. Similarly, by Lemma \ref{lemma:iffstatement}, if $\pi$ has an agreement tree, then for each position $\pi^A$ where $A \in \Gamma$, it has an agreement tree. (c) It is possible that no labels are left in $L$, this results a single set $A$ in $\Gamma$. The resulting position $\pi^A$ is identical to the position $\pi$, indicating that the profile $\P$ does not agree and \BuildAST\ should terminate.

The above arguments stay consistent for each position $\pi$ \BuildAST\ would process and generate. If profile $\P$ agrees, then it is straightforward that $\initPos$ has an agreement tree. By Lemma \ref{lemma:iffstatement} every successor of $\initPos$ has an agreement tree. Then every successor of $\initPos$ is pushed in the task queue and will be processed by \BuildAST\ later. Repeatedly executing the algorithm \BuildAST\ on every successor position generated from the predecessor position would successfully build up a super agreement tree $\T$ for $\P$. Otherwise, the algorithm would terminate immediately when disagreement is detected.

\end{proof}


%\section{Implementation Details}
%In this section, we present some details for implementations and brief discussions on time complexity issues. 

%\subsection{Additional Data Structures}

%As described in section \ref{sec:highlevel}, $\Pi$ is a queue that stores every position $\pos$ that shall map to the agreement tree \T. This queue allows \BuildAST\ to build up agreement tree \T\ in the breadth-first manner. In the inner while loop at Line \ref{algo:todoBegin}, we design another queue \Group\ that is used for keeping tack of all connected components that can be grouped together.

%\BuildAST\ plays with connected components throughout the entire life. For each connected component $W$, we associated it with a collection of sets that keep track of child labels from present trees. If $V(W) \cap V(\T_i) = \emptyset$, then $W$ would not store any child labels from that tree $\T_i$. Let $child_i$ be the child set storing child labels from tree $\T_i$. Set \Todo\ and \Remain\ are used to store connected components that are related to a position $\pos$. Both sets are active throughout the lifetime of computing successors for a position $\pos$. If $|W.child_i| \ge 2$ for any $i$, then $W$ is placed into \Todo. Otherwise, if $|W.child_i| = 1$ for some $i$, we add $W$ into \Remain.

%A position $\pos$ is not only a tuple of labels but also stands for a collection of connected components. Initially, the only connected component formed by all input trees is the component correlated to $\pos$. After computing the successors, the original component is split up and each successor is responsible for a subset of subcomponents. To achieve this, \BuildAST\ maintains some extra data structures:

%\begin{itemize}
%\item $\pos.\New = \{(v, i) : v = \pos_i $ and v firstly appears in $\pos\}$. By definition, $\initPos.\New = \{(v, i) : v = r(\T_i)$, $i \in [k]\}$. Later on, given a position $\pos$ and one of its successor $\pos'$, $\pos'.\New = \{(v, i) : v = \pos'_i$, $\pos'_i \neq \pos_i$ and $v \neq \perp\}$.
%\item $\pos.\Suspend = \{(v, i) : v = \pos_i$ and $v$ is not fully exposed$\}$. If a label $l$ appears in multiple trees, all entries $(l, i)$ will be removed from $\pos.\Suspend$ for some $\pos$ when $l$ is fully exposed.
%\item $\pos.\Todo = \{W : \exists i, |W.child_i| \ge 2, V(W) \cap V(\T_i) \neq \emptyset\}$.
%\item $\pos.\Remain = \{W : \forall i, |W.child_i| = 1, V(W) \cap V(\T_i) \neq \emptyset\}$.
%\end{itemize}

%Intuitively, a position $\pos$ is bond with a collection of connected components from $\pos.\Todo$ and $\pos.\Remain$, these components are not physically connected. If there exists a component $W$ such that $|W.child_i| \ge 2$ and another component $W'$ such that $W'.child_i \neq \NULL$, instead of physically relink $W$ and $W'$ together, we simply mark the successor $\pos'$ correlated to these two components at index $i$ with $\pos_i$ to make them conceptually connected. Suppose $\pos_i$ was from $\pos.\New$, then $\pos$ stays in the successor $\pos'$ and will not be a new label anymore. Thus \BuildAST\ will not repetitively delete $\pos_i$. 

%If a label $l = \pos_i$ is a new label, and \BuildAST\ plans to take it to process. When $l$ is tested to be not fully exposed, then it will be temporarily moved to set $\pos.\Suspend$, $l$ will be processed until it is fully exposed. To make a query of whether label $l$ is fully exposed, we keep a map structure $\Expose : l \rightarrow S$ where $S = \{i : l \in X_i\}$. Initially, each set $S$ is empty. Index $i$ will be add to $S$ of label $l$ when label $l$ at index $i$ is a new label. \BuildAST\ also maintains a count field for each label $l$, namely \textit{count}, representing how many trees $l$ is in. When $l.count = |\Expose(l)|$, label $l$ is fully exposed, otherwise it is not.

%Line \ref{algo:mergeSibling} requires to find other components that may contain any sibling of a label $l$ in tree $\T_i$. To achieve the goal efficiently, we can take advantage of another map structure $\lambda : l^P_i \rightarrow C$ where $l^P_i$ is parent label of $l$ in tree $\T_i$ and $C = \{W : V(W) \cap Ch_{\T_i}(l^P_i) \neq \emptyset$, $l \in X_i\}$. This mapping can be updated when a component $W$ is split up into two subcomponents $W_S$ and $W_L$. $W_S$ is updated by moving correlated information from $W$ to it, while the remaining $W$ becomes $W_L$. Similarly, Line \ref{algo:mergeSameLabel} may require the same operations to find all components correlated to a label $l$. When a label $l$ $\in$ $X_i$ stays in a position $\pos$, other label $l$ $\in$ $X_j$, $j \neq i$ must stay in position $\pos$ as well. The same structure can help find all components that contain children of label $l$ in another tree $\T_j$ efficiently.

%Additionally, local sets can be applied to \BuildAST\ to avoid visiting the same components or the child sets regarding to the same tree $\T_i$ after successor $\pos'$ contains $\pos'_i = \pos_i$.

%\subsection{An example}
%To help explain how the data structures work, we discuss some steps for the example we presented in this paper. Each component $W_i$ is denoted for the purpose of discuss.

%This example consists of a profile \P\ with four X-trees, namely, $\T_1$, $\T_2$, $\T_3$, $\T_4$, shown in Figure \ref{fig:profile}. By assumption, all fours are initially connected, and the figure below shows the single component created with them.
%\begin{figure}[ht]
%\centering
 % \includegraphics[scale=0.6]{charts/initial_component.jpeg}
  %\caption{The initial component $W_1$ formed by input profile $\P= \{\T_1, \T_2, \T_3, \T_4\}$.}
  %\label{fig:initialcomponent}
%\end{figure}

%Correspondingly, the position $\pos$ correlated to $W_1$ is $[1,2,g,4]$ and $\pos.\New = \{(1,1),(2,2),(g,3),(4,4)\}$. $W_1.\Todo$ and $W_1.\Remain$ are empty. Handled by Line \ref{algo:deleteBegin} to \ref{algo:deleteEnd}, \BuildAST\ firstly out that label $1, 2$ and $4$ are fully exposed. Due to label $g$ is not fully exposed, $(g, 3)$ is then added to $\pos.\Suspend$. Label $g$ will not be brought back until label $g$ in $\T_2$ is exposed. As all four labels are new labels, all child sets of $W_1$ need to be updated. As the result, $W_1.child_1 = \{5,d\}$, $W_1.child_2 = \{b,c,g\}$, $W_1.child_3 = \{k,7,f\}$ and $W_1.child_4 = \{i,j,l\}$. Fully exposed labels $1$, $2$ and $4$ and edges incident on them are deleted from $W_1$, resulting a set of subcomponents $W_2$, $W_3$, $W_4$ and $W_5$, shown in the figure \ref{fig:resultofinitial}.
%\begin{figure}[ht]
%\centering
 % \includegraphics[scale=0.6]{charts/result_of_initial.jpeg}
%  \caption{The resulting components after deleting label 1, 2 and 4 from $W_1$.}
%  \label{fig:resultofinitial}
%\end{figure}

%While deleting each label, new components may be created because the graph is no longer connected. Child sets together with some data structures are updated at this point. As a result, $W_2.child_1 = \{5\}$ and $W_2.child_2 = \{b,c\}$. Because of $|W_2.child_2| = 2$, $W_2$ would trigger merging some components back together. Thus $W_2$ is added into local set \Todo. $W_3$ is added into set \Remain, because $W_3.child_1 = \{d\}$. $W_4$ is placed into \Todo\ as $W_4.child_2 = \{g\}$, $W_4.child_3 = \{k,7,f\}$ and $W_4.child_2 = \{i,j\}$. Lastly, $W_5$ is in \Remain\ because $W_5.child_4 = \{l\}$.

%Line \ref{algo:todoBegin} to Line \ref{algo:todoEnd} will take care of grouping $W_2$, $W_3$, $W_4$ and $W_5$ back together, if possible. Due to $W_2$ may trigger merging, \BuildAST\ may start to compute one of successors $\pos'$ with $W_2$. By scanning over each child set of $W_2$, $\pos_1 = 5$ and $\pos'_2 = 2$ because there are two labels from $\T_2$ in the same component. Since $W_4$ contains another sibling of labels in $W_2.child_2$, $W_4$ is grouped with $W_2$ and scanned. $\pos'_2$ will not be changed as it has already been the parent of label $g$. $\pos'_3 = g$ and $\pos'_4 = 4$ correspondingly as their children are not scattered into different components. $W_5$ is the component that is grouped with $W_2$ and $W_4$ because label $l$ is the sibling of labels in $W_4.child_4$. Meanwhile, $W_2$ and $W_4$ are added to $\pos'.\Todo$ and $W_5$ is placed into $\pos'.\Remain$.

%As the result, components $W_2$, $W_4$ and $W_5$ are grouped together. And the correlated position $\pos' = [5, 2, g, 4]$. To note that although these three components are not physically connected, they are grouped to be components of $\pos'$. What is important at this step is to distinguish new labels from all labels in $\pos'$. Label $2$, $g$ and $4$ stay unchanged, and this means that these nodes should not be deleted again when \BuildAST\ takes $\pos'$ as input. The only new node is label $5$ from tree $\T_1$, and it is updated in $\pos'.\New$ and label $(g, 3)$ is now in $\pos'.\Remain$. Upon to this point, a successor of $\pos$ is done.

%There is another component $W_3$ being left in the $\Remain$. Line \ref{algo:remainBegin} to Lind \ref{algo:remainEnd} scan over the only child set of $W_3$ and compute another successor $\pos'' = [d,,,]$ of $\pos$. $\pos'$ and $\pos''$ correspond to two subtrees of $\pos$ in \T.

%Finally, Line \ref{algo:createNode} creates a new node with label set $\{1\}$ as a root in \T\ for $\pos$. 

\section{Running Time Analysis}

\begin{claim}
\BuildAST\ successfully builds up an agreement supertree for an input profile $\mathcal{P} = \{\T_1, \T_2, \dots , \T_k\}$ in $\mathcal{O}(M_p(\Sigma_{i \in [k]} d^{\T_i}_{max}))$ time, where $M_p = n \times k$ and $d^{\T_i}_{max}$ is the maximum degree of a node in tree $\T_i$.
\end{claim}

\begin{proof}
In Algorithm \ref{algo:buildast}, initialization at Line \ref{algo:initialization} mainly creates a connected component and the minimal spanning tree used in \textit{HDT}. Constructing the connected component requires to scan every edge and node in the input trees, and creating minimal spanning tree only needs to walk through the graph once with Depth-First Search. Both of them need at most $\mathcal{O}(M_P)$ time to scan over the whole graph. Besides, computing the count of appearance of each node also takes the same amount of time. Besides, computing the initial position \initPos\ and update new node set of it take $\mathcal{O}(k)$ time as initially all roots of the input trees are used in the position and all of them are new nodes. Therefore, initialization stage takes at most $\mathcal{O}(M_p)$ time in total.

When handling each position $\pos$ between Line \ref{algo:deletionstart} to \ref{algo:deletionend},  \BuildAST will delete every newly fully exposed nodes in the position $\pos$ and edges incident on these nodes. As we take advantage of $HDT$ data structure, deleting such an edge from the graph takes amortized $\mathcal{O}(\log^2M_p)$ time, and querying whether two endpoints are still connected after the deletion takes $\mathcal{O}(\log M_p)$ time, where $M_p = n \times k$ is approximately the size of the graph. Throughout the entire execution of \BuildAST, every edge in the graph is only deleted and queried once, thus deletions and queries take only $\mathcal{O}(M_p \log^2M_p)$ time in total. As every node in the graph is only visited once, therefore it is bounded with $\mathcal{O}(M_p)$ time. If a label appears multiple times, then this label may be suspended and then exposed when it is fully exposed. To note that each node will only be suspended once, thus it takes $\mathcal{O}(M_p)$ time as well.

While deleting an edge from the graph, a connected component may be split up into two smaller connected components, namely $W'$ and $W$, then we need to scan over the smaller one and update the child sets for them. Without lose of generality, we assume the $W'$ is the smaller one. Due to $|V'| \leq |V|$, the total time spent on scanning the smaller connected components is $\mathcal{O}(M_p \log M_p)$. Due to each node $v$ can be in at most $\mathcal{O}(\log M_p)$ connected components, moving a non-labeled node from original child set to new set takes $\mathcal{O}(\log M_p)$ time in total while moving a labeled node takes $\mathcal{O}(k \log M_p)$ as a label may appear in at most $\mathcal{O}(k)$ trees. Respectively, processing the entire graph takes $\mathcal{O}((M_p - n)\log M_p + nk \log M_p) = \mathcal{O}(M_p \log M_p)$ time.

We then perform the analysis on Algorithm \ref{algo:mergefunction}(Line \ref{algo:mergecomponents} in Algorithm \ref{algo:buildast}). From Line \ref{algo:multisuccessorsstart} to \ref{algo:multisuccessorsend}, the algorithm intends to compute a set of successors for a position $\pos$. These lines are designed to "reconnect" a set of connected components conceptually as to preserve the LCA mappings from the original trees. The algorithm fetches an index $i$ from set \Todo, which was known that $Ch_{\T_i}(\pi_i)$ violates condition C1 and thus needs to be "reconnected". As grouping a set of components that contains $Ch_{\T_i}(\pi_i)$ is required, it walks through every connected component or group that contains $Ch_{\T_i}(\pi_i)$ and searches every child set in these components for potential indices that will be handled later. Therefore, for each index $i$, it takes at most $\mathcal{O}(k \times d_{\pi_i})$, where $d_{\pi_i}$ is the out-degree of node $\pi_i$ in tree $\T_i$. To note that the if block starting at Line \ref{algo:multilabelupdate1}, \ref{algo:multilabelupdate2} and \ref{algo:multilabelupdate3} are responsible for gathering the same label from different trees together, and they would be executed at most once if those parts are entered. To argue the running time of these blocks, we observe that these blocks will be entered when a certain label $l$ is firstly recreated at the successor position. This may require to scan over some of the edges of $\pi_{r'}$ again to group all the connected components.  Therefore, the whole Algorithm \ref{algo:mergefunction} would spend at most $\mathcal{O}(\Sigma_{i \in K} kd_{\pi_i})$ time in total, where $K \subseteq [k]$.

Algorithm \ref{algo:singlefunction} is responsible for computing successors for the rest of connected components in \Comp. Since these components were not grouped with any other components, then they must not have those index $i \in K$. So Algorithm \ref{algo:singlefunction} spends at most $\mathcal{O}(\Sigma_{i \in K'} d_{\pi_i})$ time on scanning over these components, where $K' = [k] \setminus K$. It is reasonable that $\mathcal{O}(\Sigma_{i \in K'} d_{\pi_i}) \leq \mathcal{O}(\Sigma_{i \in K'} kd_{\pi_i})$ and $d_{\pi_i} \leq d^{\T_i}_{max}$,. Therefore, Algorithm \ref{algo:mergefunction} and \ref{algo:singlefunction} cost $\mathcal{O}(k\Sigma_{i \in [k]} d^{\T_i}_{max}) $ time in total. Due to the number of successors is bounded by the size of agreement tree $\T$, $\mathcal{O}(n)$, computing successors costs a total $\mathcal{O}(nk\Sigma_{i \in [k]} d^{\T_i}_{max})$ time.

To summarize, the execution of \BuildAST\ on a profile \P\ takes $\mathcal{O}(M_p(\Sigma_{i \in [k]} d^{\T_i}_{max}))$ time in total.
\end{proof}
